DeltaZip: Efficient Serving of Multiple Full-Model-Tuned LLMs

Fine-tuning large language models (LLMs) greatly improves model quality for downstream tasks. However, serving many fine-tuned LLMs concurrently is challenging due to the sporadic, bursty, and varying request patterns of different LLMs. To bridge this gap, we present DeltaZip, an LLM serving system that efficiently serves multiple full-parameter fine-tuned models concurrently by aggressively compressing model deltas by up to 10x while maintaining high model quality. The key insight behind this design is that fine-tuning results in small-magnitude changes to the pre-trained model. By co-designing the serving system with the compression algorithm, DeltaZip achieves 2x to 12x improvement in throughput compared to the state-of-the-art systems.

==> algorithms/fmzip.tex <==
\begin{algorithm}
    \caption{\texttt{\projectname} algorithm, modified from \texttt{SparseGPT} algorithm. \\Assuming a $N$-layer neural network where each layer is a matrix, we quantize and prune the layer matrix $\mathbf{w}_q$ to $p\%$ and $k$ bits given inverse Hesian $\mathbf{H}^{-1}_q=(2\mathbf{X}\mathbf{X}^T+\lambda\mathbf{I})^{-1}$. \\ We perform quantization and pruning block by block with a block size $B$ and adaptive mask selection blocksize $B_s$\\ The weight matrix from base model is given by $\mathbf{w}_b$ and we ignore the subscript for layer as we always take the same layer as $w_q$}\label{alg:fmzip_obs}
    \begin{algorithmic}
    \For{$n=0,1,2,\cdots, N$}
    
    \State $\mathbf{M} \gets \mathbf{1}_{d_{\text{row}}\times d_{\text{col}}}$ \Comment{Binary Pruning Mask}
    \State $\mathbf{Q} \gets \mathbf{0}_{d_{\text{row}}\times d_{\text{col}}}$ \Comment{Quantized Delta}
    \State $\mathbf{H}^{-1} \gets \text{Cholesky}(\mathbf{H}^{-1})^T$
    \State $\Delta = \mathbf{w}_n - \mathbf{w}_b$
    \For{$i=0,B,2B,\cdots$}
        \For{$j=i, \cdots, i+B-1$}
            \If{$j$ mod $B_S=0$}
                \State $\mathbf{M}_{:,j:(j+B_s)} \gets $ mask of $(1-p)\%$ weights $\Delta_c\in \Delta_{:, j:(j+B_s)}$ with largest $w_c^2/[\mathbf{H}^{-1}]_{cc}^2$
                \State $\mathbf{Q}_{:, j:(j+B_s)} \gets \text{quant}(\Delta_{:, j:(j+B_s)})$
            \EndIf
            \State $\mathbf{E}_{:, j-i} \gets (\Delta_{:,j} - \mathbf{M}_{:,j}\cdot \mathbf{Q}_{:,j}) / [\mathbf{H^{-1}}]_{jj}$ \Comment{Compression Error}
            \State $\mathbf{E}_{:, j-i} \gets (1-\mathbf{M_{:,j}})\cdot \mathbf{E}_{:,j-i}$
            \State $\Delta_{:,j:(i+B)}\gets \Delta_{:, j:(i+B)} - \mathbf{E}_{:, j-i}\cdot \mathbf{H}^{-1}_{j, j:(i+B)}$
        \EndFor
        \State $\Delta_{:, (i+B):}\gets \Delta_{:, (i+B):} - \mathbf{E}\cdot \mathbf{H}^{-1}_{i:(i+B), (i+B):}$
    \EndFor
    \State $\tilde{\mathbf{w}}_q \gets \mathbf{Q} \cdot \mathbf{M}  \textcolor[blue]{+\mathbf{w}_b}$ \Comment{Reconstructed Weight}
    \State $\mathbf{Y}=\tilde{\mathbf{w}}_q \mathbf{X}$ as input of next layer.
    \EndFor
    \For{$n=0,1,2\cdots, N$}
    \State pack and store $\mathbf{Q\cdot M}$ of layer $n$.
    \EndFor
    \end{algorithmic}
\end{algorithm}

==> tables/3b-quality-full.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
      \hline
      Type & Config & Ratio & NI-151 & NI-152  & NI-372 & NI-380 & NI-523 & NI-936 & NI-1308 \\
      \hline
      \multicolumn{10}{|c|}{Base Model: OpenLlama-3B-v2}\\
      Base & - & - & 58.61 & 56.69 & 0.15 & 56.92 & 0.84 & 45 & 17.76\\
      Uncompressed & - & 1 & 100 & 100  & 97.84 & 83.38 & 75.23 & 80.07 & 76.07 \\
      SparseGPT & 4 bits, 0\% & 4.27 & 75.98 & 98.07 & 97.92 & 81.83 & 72.51 & 76.90 & 77.13 \\
      SparseGPT & 4 bits, 75\% & 5.29 & 7.08 & 7.77 & 90.14 & 62.50 & 0 & 55.42 & 52.04 \\
      \projectname & 4 bits, 0\% & 4.77 & 100 & 100 &  97.92 & 83.29 & \textbf{73.51} & 79.98 & \textbf{77.90} \\
      \projectname & 4 bits, 75\% & 6.53 & 100 & 100 &  98.22 & 82.90 & 68.43 & \textbf{80.60} & 77.82 \\
      \projectname & 2 bits, 75\% & 11.32 & \textbf{100} & \textbf{100}  & \textbf{98.30} & \textbf{83.67} & 69.89 & 79.67 & 78.67 \\
      % LoRA & r=8 & 200 & 86.38 & 93.15 & 0.69 & 65.69 & 67.84 & 63.46 & 55.07 \\
      % LoRA & r=128 & 13.08 & 85.76 & 94.30  & 0.53 & 65.53 & 65.07 & 61.38 & 52.38 \\ 
      \hline
      \multicolumn{10}{|c|}{Base Model: Pythia-2.8B-deduped}\\
      Base & - & - & 58 & 55.23 & 0 & 57 & 0.76 & 44 & 18.07 \\
      Uncompressed & - & 1 & 100 & 99.15 & 94.23 &  79.61 & 76.92 & 73.23 & 73.76 \\
      SparseGPT & 4 bits, 0\% & 3.77 & 100 & 98.61 &  93.53 & 77.13 & 77.59 & 71.28 & 72.74 \\
      SparseGPT & 4 bits, 75\% & 4.44 & 99.15 & 90.99  & 65.12 & 54.19 & 71.82 & 57.12 & 50.80 \\
      \projectname & 4 bits, 0\% & 4.25 & 100 & \textbf{99.38} & \textbf{93.99} & \textbf{78.75} & 76.90 & 71.74 & \textbf{74.13}
       \\
      \projectname & 4 bits, 75\% & 6.06 & 100 & 98.30 & 91.22 & 78.67 & \textbf{81.37} & 70.74 & 72.74 \\
      \projectname & 2 bits, 75\% & 9.74 & \textbf{100} & 98.38 & 91.76 & 78.29 & 79.52 & \textbf{71.82} & 72.20 \\
      % LoRA & r=8 & 167.74 & 91.84 & 91.53 & 4.07 & 63.76 & 78.53 & 52.15 & 50.92 \\
      % LoRA & r=128 & 10.81 & 92.61 & 91.23 & 4.23 & 60.23 & 78.30 & 49.92 & 50.46 \\
      \hline
    \end{tabular}
    \caption{Model Quality of \projectname vs. Uncompressed vs. SparseGPT on various natural instruction datasets.}
    \label{tab:model_accuracy_3b_full}
  \end{table*}

==> tables/3b-quality-simplified.tex <==
\begin{table}[!ht]
  \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}llllll@{}}
\toprule
Type     & Config   & Ratio & NI-372         & NI-380         & NI-523         \\ \midrule
\multicolumn{6}{c}{\textbf{Base Model: OpenLlama-3B-v2}}                                \\ \midrule
Base     & -        & -     & 0.15           & 56.92          & 0.84           \\ \midrule
FP16     & -        & 1     & 97.84          & 83.38          & 75.23          \\ \midrule
Baseline & 4b,75\%  & 5.29  & 90.14          & 62.50          & 0              \\ \midrule
Ours     & 4b,75\%  & 6.53  & 98.22          & 82.90          & 68.43          \\ \midrule
Ours     & 2b,75\%  & 11.32 & 98.30 & 83.67 & 69.89          \\ \midrule
\multicolumn{6}{c}{\textbf{Base Model: Pythia-2.8B-deduped}}                            \\ \midrule
Base     & -        & -     & 0              & 57             & 0.76           \\ \midrule
FP16     & -        & 1     & 94.23          & 79.61          & 76.92          \\ \midrule
Baseline & 4b, 0\%  & 3.77  & 93.53          & 77.13          & 77.59          \\ \midrule
Baseline & 4b, 75\% & 4.44  & 65.12          & 54.19          & 71.82          \\ \midrule
Ours     & 4b, 0\%  & 4.25  & 93.99 & 78.75 & 76.90          \\ \midrule
Ours     & 4b, 75\% & 6.06  & 91.22          & 78.67          & 81.37 \\ \midrule
Ours     & 2b, 75\% & 9.74  & 91.76          & 78.29          & 79.52          \\ \bottomrule
\end{tabular}
}

% baseline == sparsegpt on whole model
  \caption{Model Quality of \projectname vs. Uncompressed vs. SparseGPT on various natural instruction datasets.}
  \label{tab:model_accuracy_3b_simplified}
\end{table}
